Compressed Representations of Conjunctive Query Results

Relational queries, and in particular join queries, often generate large output results when executed over a huge dataset. In such cases, it is often infeasible to store the whole materialized output if we plan to reuse it further down a data processing pipeline. Motivated by this problem, we study the construction of space-efficient compressed representations of the output of conjunctive queries, with the goal of supporting the efficient access of the intermediate compressed result for a given access pattern. In particular, we initiate the study of an important tradeoff: minimizing the space necessary to store the compressed result, versus minimizing the answer time and delay for an access request over the result. Our main contribution is a novel parameterized data structure, which can be tuned to trade off space for answer time. The tradeoff allows us to control the space requirement of the data structure precisely, and depends both on the structure of the query and the access pattern. We show how we can use the data structure in conjunction with query decomposition techniques, in order to efficiently represent the outputs for several classes of conjunctive queries.

==> algorithm.tex <==
\section{Other Compressed Representations}

In this section, we present some results for \pcq s that are not full, \ie 
$\bx_\sigma \cup \bx_\pi \neq \set{x_1, \dots, x_n}$. This creates
additional challenges, since we require the output must be enumerated 
such that there are no duplicates. Allowing for duplicate values makes the
problem as easy as enumerating full \pcq s, since we can simply project out
the necessary attributes before we output the tuple.

%\begin{lemma} \label{lemma:2path}
%The 2-path query can be compressed with size $O(|R_1| \cdot |R_2| / \delta^2)$ and delay $O(\delta)$, for every $1 \leq d \leq \min \{|R_1|, |R_2|\}$.
%\end{lemma}
%
%\begin{proof}
%We distinguish 3 different types of output tuples. The {\em left-light} tuples $(a,c)$ are the ones for which $d_{R_1}(a) \leq \delta$. The {\em right-light} tuples $(a,c)$ are the ones for which $d_{R_1}(a) > \delta$ and $d_{R_2}(c) \leq \delta$. The remaining tuples are called {\em heavy}.
%
%The first observation is that the heavy tuples are at most $(|R_1|/\delta)\cdot (|R_2|/\delta)$, so we can compute and store them as they are with space $O(|R_1| \cdot |R_2| / \delta^2)$. We also store for each value of variable $x_1$ (and of variable $x_2$) whether it participates in an answer or not.
%
%It is easy to see that we can enumerate the heavy tuples with constant delay. As for the left-light tuples, we go over every value $a$ of variable $x_1$ that participates in an answer. For each $a$, there are at most $\delta$ values, say  $b_1, \dots, b_\delta$ such that $R_1(a, b_i)$ is a tuple. For each $b_i$ we keep a pointer on the list of tuples of the form $R_2(b_i, *)$ (we assume that $R_2$ is ordered); we thus have at most $\delta$ pointers (initialized say to -1 position). Our goal is to output all the tuples $(a, c)$ in increasing order of the $c$-value. The key step is the following: we go over the next positions of the pointers, find the minimum value (say $c_{min}$), and move all pointers with value equal to $c_{min}$: we also output $(a, c_{min})$. This takes time $O(\delta)$, since considering each pointer requires constant time. We do the same for the right-light tuples.
%\end{proof}

%\begin{proof}
%We distinguish between two different types of output tuples. We say that an output tuple $P(a,b)$ is {\em heavy} if there exists $c$ such that $R(a,c), S(c,b)$,  $deg_S(c) \geq |S|/ d$ and  $deg_R(c) \geq |R|/d$. An output tuple is {\em light} otherwise.
%
%We use the observation that the number of light tuples is at most $2 |R| \cdot |S| /d$. Thus, we can store these using space $O(|R| \cdot |S| / d)$. The heavy tuples can be too many, so we do not store heavy tuples explicitly. Instead, for each value $c$ such that  $deg_S(c) \geq |S| /d$ and $deg_R(c) \geq |R|/d$, we store two lists of tuples: $A_c = \{ a \mid (a,c) \in R \}$ and $B_c = \{ b \mid (c,b) \in S \}$. We need only $O(|R| + |S|)$ space for this. We are careful to store each list using some order on the $a$ and $b$ values. 
%
%To enumerate the results, we first enumerate the light tuples: this needs only constant delay. For the heavy tuples, we output the results by computing all results of the cartesian product $A_c \times B_c$ for every $c$. Note however that a tuple $(a,b)$ can appear as the output for every $c$. To resolve this, we will produce the tuples in alphabetical order; for this, we need to keep $L$ pointers, and the next tuple will take time $O(L)$ to be output. Notice now that there can be at most $d$ values of $c$, so the delay will be $O(d)$.
%\end{proof}

%Notice that if we pick $d=1$, then we essentially store all the output results. If say $m = |R_1| = |R_2|$, we can obtain $O(\sqrt{m})$ delay with $O(m)$ space. Can we do better? It is not clear!
%
%
%\subsection{Enumerating path end points}

Our results in this section are focused on the path query $P_n$.
We will start with the query $P_2(x_1,x_2,x_3) = R_1(x_1, x_2), R_2(x_2, x_3)$,
which is just the simple join, and consider compressed representations for
$(\set{x_1}, \set{x_3})$. A compressed representation for $(\set{x_1}, \set{x_3})$ gives
directly a compressed representation for $(\set{}, \set{x_1, x_3})$ with the same space/delay
tradeoff, since we can simply iterate over all values that $x_1$ can take, and for each value 
enumerate the corresponding enumeration problem for $(\set{x_1}, \set{x_3})$.
We show the following size-delay tradeoff:
%
%In this section, we look at path queries of the form $P_k(a_1, x_{k+1}) = R_1(a_1 ,x_2), R_2(x_2, x_3), \dots, R_k(x_k, x_{k+1})$ for some $a_1$ in the domain of $x_1$. In other words, given a specific value $a_1$, we wish to enumerate over all end points in the path query such that there is a join path between all tuples of the form $R_1(a_1, *)$ and all other relations.
%
%For simplicity of exposition we describe our ideas on the 2-path query $P_2(a_1)$ and then generalize it to arbitrary (but fixed) number of relations. 



\begin{proposition} \label{lemma:2pathendpoint}
There exists a compressed representation of the path query $P_2$ that uses  space 
%
$$ S = O(|D| + |R_1| \cdot |R_2| / \delta^2)$$
and can be used to enumerate any instantiation of  the \pcq\ $(\set{x_1}, \set{x_3})$
with delay $\tilde{O}(\delta)$ for every $1 \leq \delta \leq \min \{|R_1|, |R_2|\}$.
\end{proposition}

\begin{proof}

Consider an arbitrary value $a$ in the domain of $x_1$. We classify each such $a$ as \textit{heavy} (\textit{light}) if the degree is $d_{R_1}(a) > \delta (\leq \delta)$. In order to perform the enumeration, we create two copies of the relation $R_2(x_2, x_3)$ called $R_2^{heavy}$ and $R_2^{light}$. Next, we sort relation $R_2^{light}$ by attributes in the order $x_2, x_3$ and relation $R_2^{heavy}$ by attributes in the order $x_3, x_2$.

If $a$ is a light value, there are at most $\delta$ values $b_i$ such that $(a, b_i) \in R_1$. We enumerate
the values of $x_3$ that match in increasing order as follows. At any point we remember the previously
largest value we have output so far; let is be $c_{min}$. To find the next largest value, we perform a binary
search through each list of the form $R_2^{light}(b_i, *)$ (this is possible because we sorted $R_2^{light}$ over $b_i$). Note that there are at most $\delta$ such lists, so we can find the next largest value with delay
$O(\delta \log |D|) = \tilde{O}(\delta)$.

For the \textit{heavy} tuples $(a, b_i)$, we store the following information from the pre-processing phase. For every block of $\delta$ tuples of the form $(b_j, c_k)$ in $R_2^{heavy}$, we store a bit if there exists an output $c_k$ in that block. Note that if there exists two (or more) distinct tuples with the same $c_k$ but different $b_j$ spread across two (or more) different blocks, then exactly one of them will have the bit set to $1$ and all other blocks will have $0$ bit stored unless there exists a different $c_{k'}$ that is a part of the output. It is easy to see that we have exactly $|R_2|/\delta$ blocks in total. Since we store this information only for \textit{heavy} $a$, there are at most $|R_1|/ \delta$ such values and hence, we use at most $(|R_1|/ \delta) \cdot (|R_2| / \delta)$ space. During the enumeration phase, we enumerate over a block only if it's bit is set to $1$ for a given value $a_1$ for attribute $x_1$. We iterate over a maximum of $\delta$ tuples in a block and for each tuple $(b_j, c_k)$, we can check in constant time if $(a_1, b_j)$ is a tuple in relation $R_1$. Because $R_2^{heavy}$ is sorted by $c_k$, we only need to remember the last $c_k$ we emitted as output and ensure that within a block, we do not emit the same value again. 
\end{proof}

%Note that the algorithm outlined requires $O(\delta)$ memory to store the $\delta$ pointers when enumerating \textit{light} $(a,*)$ tuples. It is easy to transform the $O(\delta)$ memory, $\delta$ delay algorithm to constant memory, $\delta \log m$ delay algorithm by using binary search to find the next $c_{min}$ across the $\delta$ lists. \\

Similarly to what we did with the triangle query, we can define a version of the problem where given an
output tuple of the form $(a_1, a_3)$, we wish to find the smallest value $a_3'$ such that $(a_1,a_3')$ is
in the output and $a_3' > a_3$. The construction of Proposition~\ref{lemma:2pathendpoint} can be used
to do this task in time $\tilde{O}(\delta)$. We denote the routine that returns such a value by 
$\mathtt{next}(a_1, a_3)$. \\

%We show a straightforward extension of the $\delta$ delay enumeration algorithm is sufficient to solve this problem. Recall that for the 2-path query enumeration algorithm, we output the end points from the pre computed stored results for all \textit{heavy} $a_1$ and dynamically find the next minimum element from the $\delta$ lists. This immediately gives us an algorithm to find the lexicographic next output. If $a_1$ is \textit{heavy}, then we can find the next smallest $o'$ output such that $o' > o$ in constant time from the stored result assuming it is sorted. For the case when $a_1$ is \textit{light}, we find the smallest value $o'$ across all the $\delta$ lists such that it is greater than $o$ by performing binary search over the lists. This can be achieved in $O(\delta)$ time using the algorithm in~\autoref{lemma:2path}. \\

Next, we generalize the algorithm to the path query $P_n$ and the \pcq\ $(\set{x_1}, \set{x_{n+1}})$.
%We will use the result from~\autoref{lemma:2pathendpoint} in our construction. 

%\begin{lemma} \label{lemma:3pathendpoint}
%The 3-path query $P_3(a_1, x_{4})$ for some $a_1$ can be compressed with size $O(|R_1| \cdot \sqrt{|R_2| |R_3|}| / \delta)$ and delay $O(\delta)$, for every $1 \leq \delta \leq \min \{|R_1|, \sqrt{|R_2| |R_3|}|\}$.
%\end{lemma}

\begin{proposition} \label{lemma:n:pathendpoint}
There exists a compressed representation of the path query $P_n$ that uses  space 
%
$$ S = O(|D| + |D|^2/ \delta^2)$$
and can be used to enumerate any instantiation of  the \pcq\ $(\set{x_1}, \set{x_{n+1}})$
with delay $\tilde{O}(\delta^{n-1})$.
\end{proposition}

%\begin{proof}
%We divide our analysis into two parts based on whether $a_1$ is \textit{light} or \textit{heavy}. If $d_{R_1}(a_1) \leq \delta_1$, then for all tuples of the form $(a_1, b_i)$, we invoke the 2-path lexicographic query enumeration algorithm $\mathtt{ENUM}_{R_2}(b_1, o_{running})$ where $o_{running}$ stores the last output. Each $b_i$ takes $O(\delta_2)$ time with space $|R_2| |R_3| / \delta_2^2$. Then, we find the minimum across the $\delta_1$ $ b_i$ and update $o_{running}$ to the global minimum. This gives us $O(\delta_1 \delta_2)$ delay algorithm. \\
%
%
%If $d_{R_1}(a_1) > \delta_1$, then there are at most $|R_1| / \delta_1$ such values. Assume that $R_1$ is sorted by $x_1$ and for a given $x_1$, all the $b_i$ are ordered such that $(a, b_1)$ comes before $(a, b_2)$ if all output $d$ values reachable from $b_1$ are not greater than those of $b_2$. We divide the tuples of $R_1$ into $|R_1| / \delta_1$ blocks such that each block contains $\delta_1$ edges. Now, for every block, we remember a bit which is set to 1 if there exists an end point that joins with the a tuple of the form $(a_1, b_i)$. This takes at most $(|R_1| / \delta_1 )^2$ space. During the enumeration phase, we only go over the blocks where the bit is set to 1. Next, for each $b_i$ in this block, we call $\mathtt{ENUM}_{R_2}(b_i, o_{running})$. Set $o_{running}$ to be the minimum of these values and emit the result. Repeat this until a block has no more elements to output. This leads to a combined delay of $O(\delta_1 \delta_2)$ with space $(|R_2| / \delta_2 )\cdot (|R_3| / \delta_2) + (|R_1| / \delta_1 )^2$. \\
%
%Setting $\delta_1 \delta_2$ to $\delta$, the space used will be minimal when $(|R_2| / \delta_2 )\cdot (|R_3| / \delta_2) = (|R_1| / \delta_1 )^2$ which finally gives us $|R_1| \cdot \sqrt{|R_2| |R_3|}| / \delta$ space for delay $O(\delta)$.
%\end{proof}



==> lowerbound.tex <==
\section{Lower Bound}

In this section, we present tight lower bounds on space requirement for enumerating tuples in \textit{star join} with delay $\delta$. We build upon the insight presented in ~\autoref{triangle} where we reduced enumerating triangles to set intersection. More specifically, we show that any data structure that pre processes $m$ sets, $S_1, \hdots, S_m$, of total size $n$ from a universe $\mathcal{U}$, requires $\Omega(n^{2-o(1)})$ space, atleast in the pointer machine model. As we will see, this directly leads us to a space lower bound for triangle enumeration. Based on these results, we conjecture that reporting set intersection $S_i \cap S_j$ in O($|S_i \cap S_j|$) in RAM model also requires $\omega(n^{2 - o(1)})$ space.

\subsection{Computation Model}

We choose \textit{pointer machine model} as the computation model to show the lower bounds. Data structures in the pointer machine model can access memory locations only by using pointers. A popular choice to prove lower bounds is to model a data structure as a directed graph $\mathcal{G}$ with each vertex having outdegree two. Every vertex is represented by two cells; one cell contains the element from $\mathcal{U}$ and the other cell points to memory location of the next vertex. Edges between the graphs are now pointers between the cells. The graph $\mathcal{G}$ has a special vertex \textit{root($\mathcal{G}$)} with the constraint that every query $q$ starts at \textit{root($\mathcal{G}$)} and explores a connected subgraph of $\mathcal{G}$. In this way, size of subgraph is a lower bound on query time (vertices in this subgraph will contain the output vertices) and size of $\mathcal{G}$ gives a lower bound on the space requirement. Pointer machine models are very attractive to prove lower bounds where query time is of the form $Q(n) + O(t)$ where $Q(n)$ represents the searching overhead using the data structure and $t$ is the output size. In ~\autoref{}, we describe how to convert query time of $Q(n) + O(t)$ into a delay result.

\subsection{Set Intersection Reporting Lower Bound}

We begin by stating a key result of the improved lower bound framework from [afshani2016data] that will be helpful in our analysis.

\begin{theorem}[\cite{afshani2016data}, Theorem 1]\label{thm:lblemma}
Let $\mathcal{U}$ be a set of $n$ input elements and $\mathcal{Q}$ a set of queries where each query outputs
a subset of $\mathcal{U}$. Assume there exists a data structure on the pointer machine that uses $S(n)$ space
and answers each query in $Q(n) + \alpha k$ time, where $k$ is the output size.
Assume (i) the output size of any query $q \in \mathcal{Q}$, denoted by $|\mathcal{U} \cap q|$, is at least $t$, for a parameter $t \ge Q(n)$
and (ii) for integers $\ell$ and $\beta$, and indices, $i_1, \cdots, i_l$,
  $|\mathcal{U}~\cap~q_{i_1}~\cap~\cdots~\cap~q_{i_{\ell}}|~<~\beta$.  Then,
   $ S(n) = \Omega\left(\frac{|\mathcal{Q}|t}{\ell \cdot 2^{O(\alpha \beta)}}\right)$.
\end{theorem}

Consider the star join query $\ast(x_1, \hdots, x_k, y) = R_1(x_1,y), \hdots, R_k(x_k,y)$. Let the cardinality of relation $R_i$ be $n_i$, $1 \leq i \leq k$.

Consider the alphabet $\Sigma = \{0, 1\}$ with $\bb$ characters. Consider a vector $\vec{x} = (x_1, \hdots, x_d)$ such that each $x_i \in \Sigma$ for some parameter $d$ to be chosen later. We define the universe $\mathcal{U}$ as the set of all possible vector $\vec{x}$. Clearly, $|U| = \bb^d$. 

Next, consider the input set $\mathcal{D} \subseteq \mathcal{U}$ of size $D$.	We partition the set of values $d$ into $k$ disjoint sets such that size of the set is $d_i = \frac{n_i d}{\sum_{j=1}^{k} n_j}$. Note that the input is $D(d_1 + \dots + d_k) = \sum_{i=1}^{k} n_i = n$

Let $\mathcal{S}^{h}_{i,j}$ denote a sub query that takes in two parameters $i,j$ such that $\mathcal{S}^{h}_{i,j} = \{\vec{x} | x_i = j, \vec{x} \in \mathcal{D}\}$ where $i \in d_h$ and $j \in \{0,1\}$ for $1 \leq h \leq k$. Then, $\mathcal{S}^{h} = \{\mathcal{S}^{h}_{i,j} | i \in d_h, j \in \{0,1\}\}$.

Define the set of queries, $\mathcal{Q}$, as  $(\mathcal{S}^{1}_{i_1,j_1}, \mathcal{S}^{2}_{i_2,j_2}, \hdots, \mathcal{S}^{k}_{i_k,j_k}) = \{\vec{x} | \vec{x} \in \mathcal{S}^{1}_{i_1,j_1} \cap \mathcal{S}^{2}_{i_2,j_2} \hdots \cap \mathcal{S}^{k}_{i_k,j_k}\}$. 
\newline
\newline
\textbf{Analysis.} We begin by counting the number of queries. Clearly, number of sub-queries for some partition $|\mathcal{S}^{h}| = \bb d_h$. So the total number of queries is $|\mathcal{Q}| = \prod\limits_{i=1}^{k} \bb d_h$


In the worst case, we need to obey the properties in~\autoref{thm:lblemma}. We satisfy these properties by carefully choosing $d$ such that size of intersection of $\ell$ queries is bounded by $\beta$. We start by the probability of fixed query matching an element from input set $\mathcal{D}$

\begin{lemma}
The probability that a given $\mathcal{S}^{h}_{i,j}$ matches a random $\vec{x}$ is $\bb^{-1}$ and probability that a fixed query outputs $\vec{x}$ is $\bb^{-k}$
\end{lemma}

\begin{proof}
Probability that a given $x_i$ in $\vec{x}$ matches a value $j$ is $\bb^{-1}$ by construction. Second part follows since $\vec{x} \in \mathcal{S}^{h_1}_{i,j}$ and $\vec{x} \in \mathcal{S}^{h_2}_{i',j'}$ are independent events. 
\end{proof}

\begin{corollary} \label{corr:expsize}
The expected output size of a query $q = (\mathcal{S}^{1}_{i_1,j_1}, \hdots, \mathcal{S}^{k}_{i_k,j_k})$ is $D/\bb^k$.
\end{corollary}

Next, we apply the Chernoff bounds to show that all queries output have a large output in order.

Let $X_i$ be an indicator random variable such that $X_i = 1$ if $\vec{x}_i \in q$, $1 \leq i \leq D$. Let $X = \sum_{i=1}^{D} X_i$. By~\autoref{corr:expsize}, $\mathbb{E}[X] = D/\bb^{k}$. Using  Chernoff bound, $\Pr[|q| > (1+\gamma )D/\bb^k ] \leq e^{ - \gamma D/3 (\bb^k) }$ for some $1 < \gamma$. Applying the union bound over all possible queries, we get \todo{shouldn't the union bound be over existence of a q with small output?} $\Pr[ \exists q,  |q| > (1+\gamma )D/\bb^k] \leq \bb^{k} (d_1 d_2 \hdots d_k) e^{-\gamma D/3 (\bb^{k})}$.

We bound this probability with a constant (say $1/3$). This gives us $3 (\bb^k) (d_1 d_2 \hdots d_k) e^{-\gamma D/3 (\bb^k)} \leq 1$ which finally gives us the constraint $D \geq c \bb^k \ln (\bb^k \prod\limits_{i=1}^{k}d_i)$. Rewriting in terms of $n_i$, we get
\begin{equation} \label{eq:1}
n_1 + \dots n_k \geq c \bb^k (\prod\limits_{i=1}^{k} d_i) \ln ( \bb^k \prod\limits_{i=1}^{k} \bb d_i)
\end{equation}

where $c$ is a positive constant. Also, by~\autoref{corr:expsize}, the output size of each query is $D/\bb^k$. To satisfy first requirement of~\autoref{thm:lblemma}.
\begin{equation} \label{eq:2}
n_i \geq \bb^k d_i Q(n)
\end{equation}

Next, we focus on satisfying second requirement of~\autoref{thm:lblemma}. Consider $\ell$ queries $q_1, \hdots, q_\ell$. Assume that intersection of $q_1, \hdots, q_\ell$ is not empty (otherwise, second requirement is already satisfied). Let $\ell_h$ denote the size of $d_h$ for sub query $\mathcal{S}^{h}_{i,j}$. Then, it must be that $\prod\limits_{h=1}^{k}\ell_h \geq \ell$ otherwise we will not be able to construct $\ell$ queries. 

\begin{lemma} \label{lemma:lpattern}
The probability that a random vector $\vec{x}~\in~\mathcal{D}$ satisfies $\ell$ sub queries is at most~$\frac{1}{\bb^l}$ and the expected number of such vectors from $\mathcal{D}$ is~$\frac{D}{\bb^\ell}$
\end{lemma}  

\begin{proof}
The events $x_i = j$ for all $\ell$ $\mathcal{S}_{i,j}$ sub queries is independent. For a fixed value $i',j$, probability that $x_i' = j$ is $1/\bb$. The result then easily follows.
\end{proof}

\begin{lemma}
The number of sets that contain $l_1, \dots, l_k$ distinct indices for $i$ in a sub query is at most $(\bb d)^{k \ell}$
\end{lemma}
\begin{proof}
Consider a sub query $\mathcal{S}^{h}_{i,j}$. The index $i$ can take exactly $d_h$ values. Therefore, the number of queries that can be formed with $\ell_h$ indices is at most $(\bb d_h)^{\ell_h}$. Taking the product for all $1 \leq h \leq k$, the total number of sub queries is  
$\prod\limits_{h=1}^{k} (\bb d_h)^{\ell_h} = \bb^{\sum l_h} \prod\limits_{h=1}^{k} d_h^{\ell_h} \leq (\bb d)^{k \ell}$ where the last inequality uses the fact that $\ell \leq \sum l_h$ and $d_h \leq d$.
\end{proof}

We apply the Chernoff bounds to bound the intersection of given $\ell$ sub queries.

\begin{lemma}
The probability that at least $\beta$ vectors satisfy $\ell$ given sub queries is at most $e^{-\gamma D/3 (\bb^\ell)}$
\end{lemma}

\begin{proof}
Let $X_i$ be an indicator random variable such that $X_i = 1$ if $\vec{x}_i \in q$, $1 \leq i \leq D$. Let $X = \sum_{i=1}^{D} X_i$. By~\autoref{lemma:lpattern}, $\mathbb{E}[X] = D/ \bb^\ell$. Using Chernoff bound, $\Pr[|q| > (1+\gamma )D/ \bb^\ell] \leq e^{- \gamma D/3(\bb^\ell)}$ for some $1 < \gamma$.
\end{proof}

 Applying the union bound over set of all possible $\ell$ sub queries, we get $\Pr[ \exists q,  |q| > (1+\gamma )D/ \bb^\ell] \leq (\bb d)^{k \ell} e^{-\gamma D/3(\bb^\ell)}$. We set this value to a fixed constant to get,
 
 \begin{equation*}
 \beta = c' \ell \ln (\bb d) (1 + \frac{1}{\gamma})
 \end{equation*}
 
where $\beta = (1 + \gamma)D/\bb^\ell$. Rewriting in terms if $n_i$, we get

 \begin{equation} \label{eq:3}
 \gamma =  c' \ell \bb^{\ell} (\prod\limits_{h=1}^{k} d_h) \ln (\bb d) / (n_1 + \dots + n_k) > 1
 \end{equation}

By~\autoref{thm:lblemma}, we have $S(n) \geq \frac{|\mathcal{Q}|t}{\ell^2 2^{O(\beta)}}$ subject to satisfying~\autoref{eq:1},~\autoref{eq:2} and~\autoref{eq:3}. Setting $\ell = \log_2{(n_1 + \dots + n_k) / \prod\limits_{h=1}^{k} d_h)}$, \\ $S(n)Q^{k-1}(n) \geq \frac{Q^k(n) \prod\limits_{i=1}^{k} (\bb d_i) \prod\limits_{i=1}^{k} (n_i)}{2^{c''\ln (\bb d) \log_2{(\sum_i n_i} / \prod\limits_{h=1}^{k} d_h)}  \prod\limits_{i=1}^{k} (n_i) }$. If we can pick parameters such that 

\begin{equation} \label{eq:4}
Q^k(n) / 2^{c'' \ln (bd) \log_2({\sum_i n_i} / \prod\limits_{h=1}^{k} d_h)} \prod\limits_{i=1}^{k} \left((n_i)(\bb d_i)^{-1}\right)  \geq (\prod\limits_{i=1}^{k} n_i)^{-\epsilon'}
\end{equation}

for some small $\epsilon'$, then we are done. Re-writing~\autoref{eq:4}, we get  

\begin{equation*}
Q^k(n) / (\bb d)^{c''' \log_2({\sum_i n_i} / \prod\limits_{h=1}^{k} d_h)}  \prod\limits_{i=1}^{k} \left(n_i (\bb d_i)^{-1}\right)  \geq (\prod\limits_{i=1}^{k} n_i)^{-\epsilon'}
\end{equation*}

Note that $\bb d = \bb (\sum_i d_i) \leq \prod_i (\bb d_i)$ and $n_1 + \dots n_k \leq n_1 n_2 \dots n_k$ \todo{state assumptions here}

This gives us,

\begin{equation*}
Q^k(n) / (\bb^k d_1 d_2 \dots d_k)^{c''' \log_2({\prod\limits_{h=1}^{k} n_i} / \prod\limits_{h=1}^{k} d_h) - 1}  \prod\limits_{i=1}^{k} n_i  \geq (\prod\limits_{i=1}^{k} n_i)^{-\epsilon'}
\end{equation*}

We set $d_i = (n_i / Q(n))^{1 - \epsilon_i}$. Since we need to satisfy ~\autoref{eq:2} for each $n_i$, we need to ensure than $Q(n) \leq min n_i$. 


\todo{re-phrase}
\begin{theorem}
Any data structure on a pointer machine that pre-processes $n$ sets and answers set intersection queries of the form $S_1 \cap S_j$ in $Q(n) + O(t)$ time requires space atleast $S(n)Q(n) = \Omega(n^{2 - \epsilon})$
\end{theorem}

\subsection{Translating Pointer Machine to Delay}

Consider a set intersection result of size $k$. A $\delta$-delay algorithm will take time $\delta k$ to output the entire result. On the other hand, pointer machine takes $Q(n) + k$ time. If $k$ is small, then time time is dominated by $Q(n)$ and if $k$ is large, then time is dominated by $k$ itself. For an output of size $k$, the delay $\delta \geq Q(n)/k$. If $k_{\text{max}}$ denotes the largest output for any set intersection query, then $Q(n) \leq \delta k_{\text{max}}$. Bounding the output of all queries to be close to $\delta$, $Q(n) \leq \delta^2$

\todo{Need to discuss this argument}


%\subsection{General triangle enumeration lower bound}
%
%In this section, we generalize the lower bound to arbitrary cardinalities of relations $R, S, T$ that participate in triangle join. Let $|R| = n_1$ and $|T| = n_2$. We issues set intersection queries from relation $S$. However, the number of set intersection queries \todo{refer same notation from sec 4?} is now lesser than $|R||T| = n_1 n_2$, i.e, $|S| = |\mathcal{Q}| \leq n_1 n_2$.
%
%\begin{lemma}
%Given relations $R, S, T$ with cardinalities greater than 0, there exists a relation (say $S$) such that $|S| \leq |R||T|$
%\end{lemma}
%
%\begin{proof}
%We show the result by contradiction. Assume that there does not exist such a relation. Then, $|R| > |S||T|, |S| > |R||T|$ and $|T| > |R||S|$. Combining all three conditions, we get $|R||S||T| > |R|^2 |S|^2 |T|^2$ which means that $0 < |R||S||T| < 1$.  This is a contradiction since cardinality of each relation is atleast one.
%\end{proof}
%
%Next, we revisit conditions in~\autoref{eq:1},~\autoref{eq:2} and~\autoref{eq:3} for the case when $|S| \leq n_1 n_2$. It is easy to see that $(bd)$ is replaced in~\autoref{eq:1} with $|S|$ and~\autoref{eq:3} remains unchanged. Note that the input is now $n_1 + n_2 = D.d$
%
%\begin{equation} \label{eq:4}
%n _1 + n_2 \geq cb^2d \ln |S|
%\end{equation}
%
%\begin{equation} \label{eq:5}
%n_1 + n_2 \geq b^2d Q(n)
%\end{equation}
%
%\begin{equation} \label{eq:6}
% \beta \geq c'l \ln (bd) (1 + \frac{1}{\gamma})
%\end{equation}
%
%Subject to the above constraints being satisfied, we can apply~\autoref{thm:lblemma} for $\ell=2$, giving us $S(n)Q(n) \geq |S|   Q^2(n) \sqrt{|S| n_1 n_2} /\sqrt{|S| n_1 n_2} (bd)^{\ell c''''}$. For constant $Q(n)$, we need to pick parameters such that $\sqrt{|S|}/\sqrt{n_1 n_2} (bd)^{\ell c''''} \geq (|S| n_1 n_2)^-\epsilon$. 
%


==> review.tex <==

\newcommand{\ans}[1]{\textbf{\em Answer. }{#1}}
\newcommand{\tbd}[1]{\textbf{\em Answer. } {\color[rgb]{0.9, 0.2, 0.0}{#1}}}
\newpage
\onecolumn

\section*{Review Changes}

We address comments from each reviewer individually as described in the following sections.

\subsection*{Reviewer 1}
\begin{enumerate}
	
\item There is some text on this in the introduction right before the "Our Contribution" paragraph, but it is not completely clear what is the difference. Perhaps the space from the Related Work section would be better used if this was explained.

\tbd{To be completed.}

\item Before "Our contributions" - this paragraph has many claims that something can not be achieved using certain techniques, but no reference is given. Are these folklore results/conjectures? Or were they proven somewhere?

\tbd{To be completed. These are statements with proof.}

\item fractional edge cover number - a citation should be added.

\tbd{To be completed.}

\item when discussing the space needed to achieve delay something should be said about pre-processing time. This becomes clear later in the paper, but on a first read it is not.

\tbd{To be completed.}

\item Reference $[9]$ has the journal missing.

\ans{This is corrected now}

\item Section $2.1$ - when defining valuations and query evaluation - although all of this is standard some more details should be given (e.g. $R_F$ is not specified at this point)

\ans{$R_F$ notations has been introduced before use.}

\item paragraph 1: $Q(x_1,...,x_\mu) = V(v(x_1),...,v(x_k))$ would imply that v is over $\{x_1,...,x_k\}$ and not only the selection variables.

\ans{The sentence has been fixed to reflect valuations only over selection variables.}

\item perhaps a more appropriate tile would be "The problem we study"/"Problem statement", or something similar.

\ans{We have changed the section heading to {\em Problem Description}}

\item Answer time, item (ii) - $O(\log |D|)$ extra memory. What is this for? Keeping pointers/indices to the database? Counting the size?

\tbd{To be completed.}

\item after Prop 1. "we can enumerate the result in constant time" - you mean delay.

\ans{The sentence is now corrected.}

\item first paragraph, defining the lexicographical order. This should be made more precise. In particular, the order is over domains, so the notation is slightly confusing.

\ans{We have introduced additional notation to clarify the total ordering for all projection variable tuples.}

\item This should be expanded to explain how enumeration/computation is performed. In particular, I did not understand what is meant in the final part with "we create three indexes...". I get that this follows from the AGM bound, but did not catch what was the intention here. Perhaps sketching both algorithms would be nice.

\ans{We have added a comment at the end of paragraph that delay guarantee comes from running worst case optimal algorithm and the three indexes are required for running the join algorithm.}

\item $u_1$ should be $u_{R_1}$ technically. Same for $u_2, u_3$.

\ans{This has been fixed.}

\item I think that the soft-O notation is not that standard, so it would be good to state why the logarithmic factors do not matter. Also, in the Introduction the big-O notation is used.

\ans{small subsection on computational model has been added.}

\item box decomposition - some intuition of what l,r, etc. are would be nice.

\tbd{To be completed.}

\item Lemma 1, although this follows from the definition mostly a short proof sketch in the appendix would be nice.

\ans{Proof has been added for completeness.}

\item defining $T(I)$ - perhaps remind the reader that $B(I)$ is the box decomposition.

\tbd{To be completed.}

\item perhaps give some intuition why (i) is important.

\tbd{To be completed.}

\item  explain $\beta_L, \beta_U$.

\tbd{To be completed.}

\item End of the proof of Proposition 5 - perhaps explain the duality with Lemma 3 explicitly here.

\tbd{To be completed.}

\item perhaps state explicitly why the unit interval is enough when w has the left child.

\tbd{To be completed.}

\item "Notice that w will be the last tuple from w..." you mean t will be the last tuple from w.

\ans{This is now fixed.}

\item "since every such node requires constant time to visit" - I did not understand this fully. Is this constant in soft-O notation (i.e. logarithmic), or am I missing something.

\ans{Reaching any node from root takes constant time in soft-O notations.}

\subsection*{Reviewer 3}

\item the construction of the dictionary:
following the fact that the data are big and cannot be stored in the main memory which are the techniques used to ensure a constant delay answer of the dictionary.

\ans{Evidence that size of dictionary can fit in main memory comes from experiments performed in~\cite{graphgen2017}. The authors show that the number of "virtual nodes" (which can be thought of as a proxy for our dictionary) fit in main memory of $64$GM RAM machine. Our data structure can potentially improve upon this as we have a more specific analysis for {\em heavy hitters}}


\end{enumerate}


==> setintersect.tex <==
\section{Fast k-Set Intersection}
\label{sec:gfsi}

In this section, we look at the problem of computing fast the intersection
of $k$ sets, where each set is chosen from a different family of sets, by
allowing a preprocessing of the input families.
We call this problem {\em Fast $k$-Set Intersection}, in short \GFSI.
For a family of sets $\mathcal{R}$, we use
the notation $\norm{\mathcal{R}} =  \sum_{i=1}^m |R_i|$ to measure
the sum of the set sizes in the family. 
Given $A \subseteq U$, where $U$ is the universe, we also define the {\em restriction} of 
$\mR$ on $A$ as $\mR \upharpoonright A = \setof{R \cap A}{R \in \mR}$. \\

\introparagraph{Problem Definition}
Formally, we are given $k$ families of sets $\mR^{1}, \dots, \mR^{k}$, where
$\mR^{i} =  \set{R^{i}_1, \dots, R^{i}_{\ell_i}}$. Every set 
$R^{i}_j$ is defined over the same universe $U$. We also denote
 $m_i = \norm{\mR^{i}}$. 
 
 An {\em intersection query} is defined as a vector of indices 
 $\mathbf{q} = (q_1, \dots, q_k)$, where $1 \leq q_i \leq \ell_i$ for
 every $i \in \set{1, \dots, k}$. The result of applying $\mathbf{q}$ is
 the set intersection $\bigcap_{i=1}^k  R^{i}_{q_i}$. Let $\mQ$ be
 any subset of the possible intersection queries.
  
The task in hand is to preprocess the families of sets, such that
we can achieve the following tasks:
%
\begin{description}
\item {\em Enumeration}: given any $\mathbf{q} \in \mQ$, enumerate all
the elements in the intersection $\bigcap_{i=1}^k  R^{i}_{q_i}$.
%
\item {\em Decision}: given any $\mathbf{q} \in \mQ$, decide whether
 the intersection $\bigcap_{i=1}^k  R^{i}_{q_i}$ is empty or not.
\end{description} 

The first problem is the {\em enumeration} version of \GFSI, and the
second is the {\em decision} version of \GFSI. In the decision version,
we want to obtain a yes or no answer as fast as possible. 
In the enumeration version of the problem, we will be interested in two
measures: (a) the total time to output the intersection, and
(b) the delay, which is the maximum time between outputting two
consecutive elements of the intersection.  

To solve this problem, we show how to construct during the preprocessing phase a 
data structure that generalizes the one proposed in~\cite{Cohen2010}. The size of the
data structure will be parametrized by $\delta$, which is a knob that controls the time/delay
and space tradeoff. \\


\introparagraph{The Main Data Structure}
%We assume that all families have the same size, \ie $m_1 = m_2 = \dots = m_k = m$.
We will  ignore for now the set of intersection queries $\mQ$ 
(or assume that it consists of all possible queries).
The main data structure is a $(k+1)$-ary tree $T$. Each node $v$ in the tree is responsible for a subset of the universe
$K(v) \subseteq U$.  For every $i=1, \dots, k$, define the restriction
$\mR^i[v] = \mR \upharpoonright K(v)$. 
If $v$ is a node at the $\ell$-th level, we say that a set $R_j^i$ is {\em heavy} for $v$ if its 
size is at least $\delta \cdot \alpha^\ell$, where $\alpha$ is a parameter we will set later. 
For every possible $\mathbf{q}$ such that 
all $q_i$ are heavy at $v$, node $v$ stores a bit that indicates whether the intersection is empty (0) 
or not (1).


We now explain how to assign $K(v)$ to each node. The root $v$ starts with
$K(v) = U$. We then perform the assignment recursively to the next levels. 
Consider some node $v$ at level $\ell$.
%
If for some $i =1, \dots, k$ we have $\norm{\mR^i[v] } \leq \delta$, the node has no children in $T$.
%
Otherwise, we partition $K(v)$ to $(k+1)$ sets $U_1, U_2, \dots, U_{k+1}$ 
%We pick any $i \in \set{1, \dots, k}$ such that $\norm{\mR^i[v] } > \delta$; 
%without loss of generality, suppose we choose $i=1$.
such that for every $j=\set{1,\dots, k}$  we have 
$\norm{\mR^i \upharpoonright U_j} \leq  \norm{\mR^i[v]} /2$. 
%In other words, we partition $U$ such that the two smaller families
%that are created will be of about equal size. 
We create $(k+1)$
children $v_1, v_2, \dots, v_{k+1}$ for $v$, and assign $K(v_j) = U_j$
for every $j=1, \dots, k+1$.

To perform the splitting, let $e_1, e_2, \dots, e_n$ be the elements of $K(v)$ in order.
For each $i \in \set{1, \dots, k}$, let $\mu_i$ be the largest index such that 
%
$$\norm{\mR^i \upharpoonright \set{e_1, \dots, e_{\mu_i-1}}} \leq  \norm{\mR^i[v]}/2.$$
%
Without loss of generality, let us assume that $\mu_1 < \mu_2 < \dots < \mu_k$.
We set  $U_1 = \set{e_1, \dots, e_{\mu_1-1}}$,
$U_2 = \set{e_{\mu_1+1}, \dots, e_{\mu_2-1}}$, and so on.
By the choice of the indexes $\mu_j$, we know that each set $U_j$ satisfies 
the property $ \norm{\mR^i \upharpoonright U_j} \leq \norm{\mR^i[v]} /2$ for
every $i=1, \dots, k$.
%Now, let $j$ be the largest index
%such that if $U_2 = \set{e_{i+2}, \dots, e_j}$, then 
%$\norm{\mR \upharpoonright U_2} \leq \norm{\mR}/2$ and 
%$\norm{\mS \upharpoonright U_2} \leq \norm{\mS}/2$. It is now easy to see that for
%$U_3 = \set{e_{j+2}, \dots, e_k}$, we must also have that 
%$\norm{\mR \upharpoonright U_3} \leq \norm{\mR}/2$ and 
%$\norm{\mS \upharpoonright U_3} \leq \norm{\mS}/2$. 
The remaining elements $e_{\mu_1}, \dots, e_{\mu_{k}}$ that have not been assigned 
to any child will be stored at node $v$ as extra elements, which we denote $L(v)$.

In addition to the tree $T$, we will construct a hash index for each set in each node, such that we can
ask for membership in constant time $O(1)$. \\

The following lemma analyzes the space requirements of the above data structure.

\begin{lemma}
The height of the tree $T$ is upper bounded by $ \log ( \min_i {m_i})$.
Moreover, the total amount of space required to store the tree $T$ is $O(\prod_i (m_i/\delta))$.
\end{lemma}

\begin{proof}
To bound the height of the tree $T$, notice that at every level, for any $i=1, \dots, k$ the size of 
 $\mR^i_v$ is reduced by half.  After $ \log (\norm{\mR^i}  /\delta)$ levels, the size of the 
sets will be at most $\delta$, so there will be no more levels thereafter.

To bound the total space, we will compute the total space for nodes at some level $\ell$.
Consider a node $v$ at level $\ell$. Since $T$ is $(k+1)$-ary, there are at most $(k+1)^\ell$ such nodes. 
At each node $v$, we need to remember the intersection result amongst only the heavy sets for
 that node $v$. By construction, there are at most $\norm{\mR^i[v]} / (\delta \alpha^{\ell})$ heavy sets corresponding to 
 the $i$-th family. Next, we observe that $\norm{\mR^i[v]}  \leq  m_i / 2^\ell$, because at every level we are cutting by half the size of  the family. Hence, the number of intersections results we need to store at node $v$ is at most
 %
 \[
 \prod_{i=1}^k \frac{\norm{\mR^i[v]}}{\delta \alpha^{\ell} }  
 \leq \left( \frac{1}{2^\ell \alpha^{\ell}} \right)^k \prod_{i=1}^k (m_i/\delta)
 \]
%(notice that we never need to store more than $|\mQ|$ intersections at a node). 
The total space $S$ for all the nodes in the tree will now be bounded as follows:
%
$$ S \leq \prod_{i=1}^k (m_i/\delta) \cdot \sum_{\ell} (k+1)^\ell (2\alpha)^{-k\ell} $$
%
Notice that for any choice of $\alpha < (k+1)^{1/k}/2$, the quantity 
$\sum_{\ell} (k+1)^\ell (2\alpha)^{-k\ell}$
is bounded by some constant.
\end{proof}

\noindent {\bf \em Computing Intersection Queries.}
We now describe how we can use the above data structure to answer intersection queries.
Suppose we are given an intersection query $\mathbf{q} = \bigcap_{i=1}^k R^i_{q_i}$.

We start from the root and proceed recursively. If at a given node $v$ (at level $\ell$) there exists some 
$i \in \set{1, \dots, k}$ such that $R^i_{q_i}$ is not heavy (\ie the size of the intersection
$R^i_{q_i} \cap K(v)$ is at most $\delta \alpha^\ell$), we can output the intersection result restricted to $K(v)$ by asking for each element of $R^i_{q_i} \cap K(v)$ whether it exists in all the other sets (using their corresponding hash table).

Otherwise, if all sets are heavy, we check the stored entry that tells us if the intersection is empty or not.
If it is 0, we stop the recursion. If it is 1, we recursively traverse the $(k+1)$ children and the $k$ extra elements in $L(v)$. For each extra element $e \in L(v)$, we check membership in the intersection by probing the hash tables of all sets.
Notice that by starting from the leftmost child, then visiting the first node in $L(v)$, then traversing the second child, and so on, we can output the elements intersection in alphabetical order.

We next provide a guarantee on the delay of the above intersection algorithm.

\begin{lemma}
We can enumerate with delay $\delta$ the intersection query $\mathbf{q} = \bigcap_{i=1}^k R^i_{q_i}$ using the tree $T$ with parameter $\delta$. 
\end{lemma}

\begin{proof}
For a given query $\mathbf{q}$, say that a node $v$ in the tree is {\em light} if there exists a non-heavy set and we have to check the hash tables for every element in the set. This will take at most $\delta \alpha^\ell$ time, if the node is at level $\ell$. Observe that we never continue traversing the subtree under a light node. A node that is not light is called {\em heavy}.

The key observation is that while we wait to output a new element in the intersection, we can visit at most $2(k+1)$ nodes at every level. Indeed, we never visit a subtree of a light node, and for each heavy node, whenever we keep recursing down the tree, we are certain that at least one of the children will have a non-empty intersection. The time we spent on each heavy node is only $O(1)$, since we just need to check the corresponding bit.
This means that we can bound the delay by 
%
$$ 2(k+1) \delta \sum_\ell \alpha^{-\ell}$$
Since $\alpha < (k+1)^{1/k}/2 < 1$ for any $k \geq 2$, the quantity $\sum_\ell \alpha^{-\ell} $ is a constant, and the delay we obtain is $O(\delta)$.
\end{proof}

\noindent {\bf \em Bounded Queries.} The data structure we designed ignores the fact that the
possible queries come from a possibly small set $\mQ$. For example, suppose $k=2$ and 
$m_1 = m_2 =m$. If we want to solve the decision version with time $\delta$, we need to use $O(m^2/\delta^2)$ space. However, if we know that only $m$ queries will be asked, we can simply store one bit per query (to indicate whether they intersect or not); this will cost only $O(m)$ space, which is better than $O(m^2/\delta^2)$ for any $\delta \leq \sqrt{m}$. We next show how to modify our initial data structure to support the fact that the possible queries we can ask come from a set $\mQ$.

The key idea is to store less of the tree $T$. To do this,
during the preprocessing step we  split the universe $U$ of $z$ values to 
$(k\beta-1)$ smaller sets $U_1, \dots U_{k\beta-1}$, such that the size of the 
restriction of each $\mR^i$ to each $U_i$ is at most $m_i/\beta$. 
We can do this by applying the same partitioning technique we used to split the elements
to the children of a node in $T$. We will show how to choose the parameter $\beta$ later.
Our modified data structure will consist of two structures:
%
\begin{enumerate}
\item For each query $\mathbf{q} \in \mQ$, we store the list of indexes 
$j \in \{1, \dots, k\beta-1\}$ such that the intersection $\bigcap_{i=1}^k R^i_{q_i} \cap U_j$ is non-empty.
This structure needs space $O(\beta |\mQ|)$.
%
\item For each $U_j$, where $j \in \{1, \dots, k\beta-1\}$, we construct 
a separate tree $T_j$ for the \GFSI\ problem that uses as inputs the restrictions 
of each family $\mR^i$ to $U_j$. Since now each family has size $m_I/\beta$, 
storing each tree requires space $O(\prod_i (m_i/\beta\delta))$. 
\end{enumerate}

The intersection algorithm now will look at the first data structure to check which trees
will produce some output and should be visited. For each such tree, it will traverse it
exactly like the vanilla algorithm. Observe that the delay guarantee remains exactly the same
as before, $O(\delta)$.

We next consider the space requirements. The total space needed by both structures is
in the order of:
%
\begin{align} \label{eq:space}
S = |\mQ| \beta + \beta \cdot \frac{\prod_i m_i}{(\beta \delta)^k}. 
\end{align}
%
To minimize the space, observe that the first function is increasing in $\beta$, and
the second is decreasing in $\beta$. Moreover, it must be that $\beta \geq 1$. Hence, 
we set $\beta$ to the maximum of 1, and the value which makes the functions intersect.
In other words,
%
$$\beta = \max \left\{ 1, \frac{\left( \prod_i m_i\right)^{1/k}}{\delta |\mQ|^{1/k}} \right\}.$$ 

If $|\mQ| \geq (\prod_i (m_i/\delta))$, $\beta=1$ and essentially the
vanilla data structure with space $O(\prod_i (m_i/\delta))$ is the best possible.
Notice that this means that the number of queries is larger than the size of the vanilla
structure, so it is too expensive to store any information about the queries.
 Otherwise, the space required becomes
%
$$ S = O \left( \frac{|\mQ|^{1-1/k} \prod_i m_i^{1/k}}{\delta} \right)$$

We can now state the main theorem of this section.

\begin{theorem}\label{thm:fksi}
Let $\mR^{1}, \dots, \mR^{k}$ be an instance of the \GFSI\ problem with $m_i = \norm{\mR^{i}}$, and
suppose the intersection queries come from the set $\mQ$. Then, we can solve 
(i) the decision version of
\GFSI\ with time $O(\delta)$, and (ii) the enumeration version of \GFSI\  with delay $O(\delta)$ with space
%
\begin{align*}
S =  
    \begin{cases}
      O \left( \prod_i (m_i/\delta) \right) & \text {if } |\mQ| \geq \prod_i (m_i/\delta) \\
      O \left( |\mQ|^{1-1/k} \prod_i m_i^{1/k} /  \delta \right)        & \text{otherwise}
    \end{cases}
\end{align*}
\end{theorem}

%We should note here that, if $m \leq \norm{\mR}/\delta$ we can slightly change the construction of the tree to only use space $m \cdot \norm{\mS}/\delta$. To do this, the intersection matrix considers pairs with all sets from $\mR$ with the heavy sets from $\mS$. Also, when we split now we need to care only about splitting $\mS$ into equal parts.



==> triangle.tex <==
\section{Compressed Representations for Full  {p}-CQs}

In this section, we present and analyze several compressed representations 
for full \pcq\ queries over several classes of CQs, including the triangle query,
Loomis-Whitney joins, star join queries and cycle queries. The key component of the
data structures we present is the data structure for the \GFSI\ problem.


\subsection{The Triangle Query} 
\label{triangle}

We begin our study with the {\em triangle query}. We start with a simple query
so that we can present the main idea behind the reduction to the \GFSI\ problem.
The triangle query is written as:
%
$$\Delta(x,y,z) = R(x,y), S(y,z), T(z,x).$$
%
Let $|D| = |R| + |S| + |T|$ be the total input size.
Recall that the task in hand is, given a \pcq\ query $q_p$ over the intermediate relation
$\Delta$, to preprocess the input
database such that we can answer any instantiation of the $q_p$ with the smallest
delay possible.
Notice that in the case of the triangle query, all boolean \pcq s can be trivially answered
in constant time $O(1)$ using only linear space $O(|D|)$. Indeed, for any \pcq\ of the 
form $(\{x\}, \{\})$, $(\{x,y\}, \{\})$ or $(\{x,y,z\}, \{\})$, we can directly store all possible
results in only linear space.

The first interesting \pcq\ query over the triangle is $q_p = (\{x,y\}, \{z\})$. This query
reflects the following task: 
{\em given constants $a,b$, enumerate the output of the
query $q_{a,b}(z) = \Delta(a,b,z)$.} 

We will create a compressed representation for this \pcq\ by reducing the problem to
the \GFSI\ problem. As a first step, we can preprocess the input data such that we remove
any tuples in the input relations that do not participate in some output tuple. 
We will use the data structure for \GFSI\ with $k=2$.  
The universe of elements will be 
%
$$U = \pi_{z} (S) \cap \pi_z (T).$$
We construct two families of sets: $\mR^S$ for $S$ and $\mR^T$ for $T$.
Let $S_b = \setof{c}{(b,c) \in S}$ and $T_a = \setof{c}{(c,a) \in T}$. Then
the families are constructed as follows:
%
\begin{align*}
\mR_S & = \setof{S_b}{b \in \pi_y(R)} \\
\mR_T & = \setof{T_a}{a \in \pi_x(R)} 
\end{align*}
%
Finally, we construct the set of queries $\mQ = R$: an intersection query corresponds 
exactly to a  tuple in $R$ and asks to enumerate the intersection $S_b \cap T_a$.
It is straightforward to observe that enumerating all triangles of the form 
$\Delta(a,b,z)$ is equivalent to computing the query $(a,b) \in \mQ$. 

\begin{proposition}
There exists a compressed representation of the triangle query $\Delta$ that uses  space 
%
$$O(|D| + \sqrt{|R| |S| |T|} /\delta)$$ 
and can be used to enumerate the \pcq\ $ (\{x,y\}, \{z\})$
with delay $O(\delta)$.
\end{proposition}

\begin{proof}
We can apply Theorem~\ref{thm:fksi} with $|\mQ| = |R|$ to obtain that for any 
delay $\delta \leq \sqrt{|S|\cdot|T|/|R|}$, we need space 
$|S| + |T| + \sqrt{|R| |S| |T|} /\delta$ for the data structure.
Observe that if the delay we are targeting is exactly $\sqrt{|S|\cdot|T|/|R|}$, then we need 
space $O(|R|)$. Clearly, we can achieve any larger delay with the same space using the
same data structure.
\end{proof}

We should not here two things.
First, if we need to achieve constant delay $\delta = O(1)$, our compressed
representation needs space $|D| + \sqrt{|R| |S| |T|}$, which matches the AGM bound
from~\cite{AGM} for the worst-case output size of the triangle query. In other words, if we want to achieve
constant delay in our task, we may as well store the exact output. 
Second, if we consider relations of equal size, $|R| = |S| = |T| = m$, then the data
structure for delay $\delta$ requires space $O(m^{3/2}/\delta)$. This gives us a
space/delay tradeoff: 
%
$$ \textsf{space} \times \textsf{delay} = O(m^{3/2}).$$

Observe that if we want to use only linear space $O(m)$, the best delay we can achieve is 
$O(\sqrt{m})$. If we want to achieve constant delay, we need space $O(m^{3/2})$.\\

We next turn our attention to other possible \pcq s over $\Delta$. It is easy to see that the
symmetrical \pcq s $ (\{x,z\}, \{y\})$ and $ (\{z,y\}, \{x\})$ can be handled in exactly the same
way as $ (\{x,y\}, \{z\})$, achieving the same space/delay tradeoff.

The same data structure can also be used for the \pcq\ $ (\{x\}, \{y,z\})$. Indeed, in order to
enumerate the output of a query of the form $q_a(y,z) = \Delta(a,y,z)$, we can simply 
enumerate the result of the queries $q_{a,b}(z) = \Delta(a,b,z)$ iteratively for every
$b$ such that $(a,b) \in R$. We can figure out which $b$'s to search for by sorting $R$ in
lexicographical order; since we have
removed any tuples that do not participate to an output, it is guaranteed that every $(a,b)$ will 
output at least one triangle. Thus, the delay remains the same, $O(\delta)$, and we need no
extra space.
The same idea can be used to enumerate with delay $O(\delta)$ the output of the full 
enumeration \pcq\  $(\{\}, \{x,y,z\})$. Here we iterate over all edges $(a,b) \in R$, and for each edge 
we enumerate $q_{a,b}$ using the data structure in the compressed representation.

\begin{proposition}
There exists a compressed representation of the triangle query $\Delta$ that uses  space 
%
$$O(|D| + \sqrt{|R| |S| |T|} /\delta)$$ 
and can be used to enumerate the \pcq s $ (\{x\}, \{y,z\})$ and $(\{\}, \{x,y,z\})$
with delay $O(\delta)$.
\end{proposition}

The proposed compressed representation gives us an additional capability. Suppose that 
the domains of the values are ordered, and this ordering is extended to an ordering over
triangles over some lexicographical ordering: without any loss of generality, let us assume 
that we have $x < y < z$. Then, we can
perform the following task with time $O(\delta)$: 
{\em given as input a triangle $\Delta(a,b,c)$, output the lexicographically next triangle}.
Indeed, note that we can construct the state of the enumeration of $\Delta(x,y,z)$ at the
point it outputs $\Delta(a,b,c)$ in time $O(\delta)$, and then because of the bounded delay
we need $O(\delta)$ more time to output the next triangle. 

\begin{corollary}
There exists a compressed representation of the triangle query $\Delta$ that uses  space 
%
$$O(|D| + \sqrt{|R| |S| |T|} /\delta)$$ 
that allows to find the lexicographically next triangle (in any order) to a given triangle
$\Delta(a,b,c)$ in time $O(\delta)$.
\end{corollary}

We can push this idea further, and
use the data structure as a form of search index (like a B+ tree) over $\Delta$. 
For instance, we can use the compressed representation to output with
delay $O(\delta)$ all the triangles that are larger than $\Delta(a_1,b_1,c_1)$ and
smaller than $\Delta(a_2, b_2, c_2)$, or all the triangles $\Delta(x,y,z)$ such that 
$x \geq a$.

%\begin{lemma}
%The triangle query $\Delta$ admits a compression scheme with size $O(|D| \beta)$ and delay  $O(\sqrt{|R|}/\beta)$, where $R$ is the smallest relation and $\beta=1, \dots, \sqrt{|R|}$.
%\end{lemma}
%
%\begin{proof}
%Let $d_R(a)$ be the degree of value $a$ of variable $x$ in the relation $R$. Let $\tau$ be a threshold value that we will determine later. 
%
%As a first step, the compression algorithm stores $R$ in a list ordered first by the $x$-attribute and then the $y$-attribute. Moreover, it creates an index such that, given a value $a$, the position to the first tuple of the form $R(a,*)$ in the sorted order is returned. It further stores an order list of the $a$ values with $d_R(a) > \tau$: let $a_1, \dots, a_\ell$ be the ordered list,  where $ \ell \leq |R|/\tau$.
%
%As a second step, the compression algorithm computes two sets of tuples: $S_{\Delta} \subseteq S$ and $T_{\Delta} \subseteq T$. $S_{\Delta}$ includes all tuples $S(b,c)$ such that there exists a triangle $\Delta(a,b,c)$ where $d_R(a) > \tau$. $T_\Delta$ includes all tuples $T(c,a)$ such that there exists a triangle $\Delta(a,b,c)$ where $d_R(a) \leq \tau$. Each tuple $(b,c) \in S_{\Delta}$ is stored together with a bit vector of size $\beta$: the $i$-th bit of the bit vector is 0 if none of the triples $(a_k, b,c)$ form a triangle, for $k= (i-1) \frac{|R|}{\tau \beta}, \dots, i  \frac{|R|}{\tau \beta}$; otherwise it is 1. Each tuple $(c, a) \in T_{\Delta}$ is also stored together with a bit vector of size $\beta$: the first bit of the bit vector is 0 if the first $\tau/\beta$ tuples of the form $R(a,*)$ do not form any triangle with $(c,a)$, otherwise it is 1, and so on.
%
%It is easy to see that the total size of the compression is then $|R| + (|S| + |T|) \beta$.
%
%The decompression algorithm has two stages:
%%
%\begin{packed_item}
%\item For every $S(b,c) \in S_\Delta$, and for every value $a$ such that $d_R(a) > \tau$: if $(a,b) \in R$ and $(c,a) \in T$, we output $\Delta(a,b,c)$.
%\item For every $T(c,a) \in T_\Delta$, we probe the index to obtain all tuples of the form $R(a, *)$: for each such tuple we check whether $(b,c) \in S$, and if so we output $\Delta(a,b,c)$.
%\end{packed_item}
%
%To show the correctness of this algorithm, consider an output triangle $\Delta(a,b,c)$. We distinguish two cases. If $d_R(a) \leq \tau$, then it must be that $T(c,a) \in T_\Delta$, and thus the triangle will be discovered by the first stage. If $d_R(a) > \tau$, then it will be that $S(b,c) \in S_\Delta$ and the triangle will be discovered during the second stage. Since the two cases are disjoint, each triangle will be output once.
%
%To bound the delay, observe that the delay in the first stage is at most $O(|R|/(\tau \beta))$. Indeed, we know by construction that each tuple $S(b,c) \in S_\Delta$ will result in an output. With the help of the stored bit vector, we can also skip any interval of the sorted list of heavy $a$-values that is bigger than $O(|R|/(\tau \beta))$. Each check needs only constant time. The delay in the second stage is at most $O(\tau/\beta)$. Indeed, we know again by construction that each tuple $T(c,a) \in T_\Delta$ will result in a triangle output. However, since $d_R(a) \leq \tau$, with the help of the stored bit-vector we can guarantee that we will output a triangle with delay at most $\tau/\beta$.
%
%
%Hence, the delay is bounded by $\max(|R|/\tau, \tau)/\beta$, and it is minimized if we choose $\tau = \sqrt{|R|}$, in which case we obtain a delay of $\sqrt{|R|}/\beta$.
%\end{proof}

\subsection{The Star Join Query} 
\label{sec:stars}

We continue our study with the class of {\em star join} queries, which are CQs of the form
%
$$ S_n(x_1,  \dots, x_n, z) = R_1(x_1,z), R_2(x_2,z), \dots, R_n(x_n, z).$$ 
%
When $n=2$, we get the simple natural join between two binary relations. The star join
is an acyclic Conjunctive Query, which means that we can enumerate the full enumeration
\pcq\  with constant delay using only linear space. Notice that any \pcq\ of the form
$(\bx_\sigma, \bx_\pi)$ such that $z \in \bx_\sigma$ can also be enumerated in constant delay
with linear space. Indeed, once the value of $z$ is fixed, we can independently search through
each relation with constant delay to output the full result. 

Thus, the interesting case is when $z \notin \bx_\sigma$. We consider first the \pcq\ 
$(\set{x_1, \dots, x_n}, \set{z})$, which corresponds to the following  task: 
{\em given as input the values $a_1, \dots, a_n$, enumerate the output
of the query $Q(z) = S_n(a_1, \dots, a_n,z)$.}

To solve this task, we resort again to using the \GFSI\ problem, as with the triangle query.
Indeed, we can construct a family $\mR^i$ for each relation $R_i$ that contains all sets of
the form $S_{a_i} = \setof{b}{(a_i,b) \in R_i} $. Enumerating the query $Q(z) = S_n(a_1, \dots, a_n,z)$
is now equivalent to asking the query $\mathbf{q} = (a_1, \dots, a_n)$. We can now apply Theorem~\ref{thm:fksi}; since the set of queries $\mQ$ can be as large as $\prod_{i=1}^n |R_i|$, we 
obtain that we can achieve delay $O(\delta)$ with space 
$O \left( |D| + \prod_{i=1}^n (|R_i|/\delta) \right)$.
We can also use the same data structure to answer the boolean \pcq\ 
$(\set{x_1, \dots, x_n}, \set{})$ in time $O(\delta)$. 

More generally, for a \pcq 
$(\set{x_{i_1}, \dots, x_{i_r}}, \bx_\pi)$, where $z \in \bx_\pi$ we can apply the  \GFSI\ construction to make only
$r$ families of sets, one for each $x_{i_j}$. We can use this data structure to obtain each
$z$-value with delay $O(\delta)$, after which we can enumerate the possible values of the 
remaining variables with constant delay. 

\begin{proposition}
Consider the star join query $S_n$, and the \pcq\
$q_p = (\set{x_{i_1}, \dots, x_{i_r}}, \bx_\pi)$, where $z \in \bx_\pi$.
Then, there exists a compressed representation of $S_n$ that uses  space 
%
%
$$O \left( |D| + \prod_{j=1}^r (|R_{i_j}|/\delta) \right)$$ 
and can be used to enumerate $q_p$
with delay $O(\delta)$.
\end{proposition}

If all relations have the same size $m$, the space bound for delay $\delta$ becomes
$O(m^r/\delta^r)$, which means that to get for example constant delay we need $O(m^r)$ space.
This bound might seem large, but there is good reason to believe that it is the best possible,
as we discuss next. \\

\noindent {\bf \em Conditional Lower Bounds.} We next look at two conjectures that give a
conditional lower bound on the space requirement for set intersection queries. These conjectures 
directly lead to a lower bound in our setting for the star query. 

\begin{conjecture} (due to~\cite{patrascu2010distance})
Consider a data structure that preprocesses sets $S_1, \hdots, S_n \subseteq [X]$ where $X = \ln^c n$ for a constant $c$. Let $\mathbf{Q}_{i,j}$ be boolean a query that returns true of $S_i \cap S_j \neq \emptyset$, and false otherwise. If $\mathbf{Q}_{i,j}$ can be answered in constant time, then the data structure takes $\tilde{\Omega}(n^2)$ space.
\end{conjecture}

This folklore conjecture is believed to be true and widely used in problems related to information retrieval 
and document indexing~\cite{Davoodi12}. An important application of the result is on strong lower bounds for exact distance oracles~\cite{cohen2010hardness}. Next, we state another conjecture for non-boolean queries.

\begin{conjecture} (due to~\cite{Davoodi12})
Consider a data structure that preprocesses sets $S_1, \hdots, S_n$ sets of size $m$ in total,
where the maximum cardinality of the sets is polylogarithmic in $m$. If the data structure can
support set intersection queries in $\tilde{O}(\delta)$ time, it requires $\tilde{\Omega}((m/k)^2)$
space, for $1 \leq \delta \leq m$.
\end{conjecture}

%\begin{conjecture} (due to~\cite{afshani2016data})
%Consider a data structure that preprocesses sets $S_1, \hdots, S_m$ with total size $n$ over some universe $\mathcal{U}$. Let $\mathbf{Q}_{i,j}$ be a query that asks for all elements in $S_i \cap S_j$. If $\mathbf{Q}_{i,j}$ can be answered in $O(|S_i \cap S_j|)$ time, then the data structure takes $\omega(n^{2 - \epsilon})$ space for some small fixed constant $\epsilon > 0$.
%\end{conjecture}

Under this conjecture the star join query for $n=2$ and equal relational sizes would require 
$\tilde{\Omega}(m^2)$ space for constant delay enumeration, and in general $\tilde{\Omega}((m/\delta)^2)$
space for $O(\delta)$ delay enumeration. Thus, assuming the conjecture is true, our space/delay
tradeoffs for the join query and equal sizes is essentially optimal.
Any data structure that does better for set intersection queries would automatically lead to a breakthrough in improving the space/delay tradeoff for star join queries and bounds for distance oracles. 
Note that such improved bounds will also improve the corresponding boolean version of the \pcq\ as well. 

\subsection{The Loomis-Whitney Join} 
\label{sec:lw}

We show here how to construct a compressed representation for bounded delay enumeration 
for the Loomis-Whitney join query:
%
\begin{align*}
LW_n(x_1, \dots, x_n)  = & S_1(x_2, \dots, x_n),  S_2(x_1, x_3, \dots, x_n), \dots, \\
& S_n(x_1, \dots, x_{n-1})
\end{align*}

Notice that the triangle query $\Delta$ is a special case of $LW_n$ for $n=3$. We show how to
construct a compressed representation for the \pcq\ $q_p = (\set{x_1, \dots, x_{n-1}}, \set{x_n})$.
Once we have this representation, we can answer all other full \pcq s that select a subset of
$\{x_1, \dots, x_{n-1}\}$. 

We will again use the machinery of the \GFSI\ data structure. We will create $n-1$ family of sets 
$\mR^i$ for each $S_i$, where $i=1, \dots, n-1$. The sets for family $\mR^1$ are of the form
$S_{(a_2, \dots, a_{n-1})} = \setof{a_n}{(a_2, \dots, a_n) \in S_1}$; the other families can be
constructed in a symmetric way. The set of queries $\mQ$ is formed as follows: for each $a_1, a_2, \dots, a_{n-1}$,
we form a query $\mathbf{q}$, where $q_1 = (a_2, \dots, a_{n-1})$, $q_2 = (a_1, a_3, \dots, a_{n-1})$,
and so on. We can bound the set of queries with $|\mQ| = |R_n|$.

Now if we just applied Theorem~\ref{thm:fksi} directly (and all relations have size $m$), 
we would obtain a space upper bound
$O(m^{2-1/k}/\delta)$ for delay $\delta$. However, we can do better by exploiting the very particular
structure of our queries. The key observation is that the space we need to store the heavy set intersections
at each node is not as large as $\prod_i (|R_i|/\delta)$, but instead can be better bounded by
$\prod_i (|R_i|/\delta)^{1/(k-1)}$. Indeed, if each set family $\mR^i$ has $|R_i|/\delta$ heavy values, by the
AGM bound the number of heavy combinations we will have will be at most $\prod_i (|R_i|/\delta)^{1/(k-1)}$.
Equipped with this new bound, we can now rewrite Eq.~\eqref{eq:space} as
%
\begin{align*} 
S = |R_n| \beta + \beta \cdot  \prod_{i=1}^{n-1} (|R_i|/\beta \delta)^{1/(n-2)} 
\end{align*}
%
which is minimized when we choose the parameter $\beta$ such that
 $\beta = \prod_{i=1}^{n-1} |R_i|^{1/(n-1)} / (\delta |R_n|^{(n-2)/(n-1)})$. The space bound
 we obtain is $\prod_i |R_i|^{1/(n-1)}) / \delta$.
 %

\begin{proposition}
There exists a compressed representation of the LW-join query $LW_n$ that uses  space 
%
$$ S = O(|D| + \prod_{i=1}^n (|R_i|^{1/(n-1)}/\delta) )$$
that allows to enumerate any instantiation of the \pcq\ $(\set{x_1, \dots, x_{n-1}}, \set{x_n})$
with delay $O(\delta)$.
\end{proposition}

We should note here two things. First, for constant delay $\delta$, the space bound matches exactly 
the AGM bound, as we would expect. Second, if all relation sizes are equal to $m$, we get the following space/delay, which generalizes that of the triangle query:
%
 $$ \textsf{space} \times \textsf{delay} = O(m^{k/(k-1)}).$$

\subsection{Path Queries}

A {\em path query} is a CQ of the following form:
%
\begin{align*} 
P_n(x_1, \dots, x_{n+1})  = & R_1(x_1, x_2), R_2(x_2, x_3), \dots, \\
& R_k(x_n, x_{n+1}).
\end{align*}
%
We show here how to obtain compressed representations for $P_n$ for any 
full \pcq\ with selection variables $\bx_\sigma = \set{x_{i_1}, \dots, x_{i_r}}$.
We will show this only for the case where relations have equal size to $m$.

We start with the case where $\bx_\sigma = \set{x_1, x_{n+1}}$, where we are 
given as input only the values for the endpoints of the path query.

\begin{proposition}
There exists a compressed representation of the path query $P_n$ that uses  space 
%
$ S = O(m^2/\delta^2)$
and can be used to enumerate any instantiation of the \pcq\ $(\set{x_1, x_{n+1}}, \set{x_2, \dots, x_n})$
with delay $O(\delta^{n-1})$.
\end{proposition}

\begin{proof}
The construction of the compressed representation uses induction. 
The path query
$P_2$ is equivalent to the star join query $S_2$. Hence, 
with space $O(m^2/\delta^2)$ we can construct a compressed representation
that achieves enumeration with delay $O(\delta)$ for $P_2$. This is the base
of the induction.

Now, consider the path query $P_{n}$. The construction works as follows.
Define $S_{a} = \setof{a_2}{(a,a_2) \in R_1}$, and 
$T_{b} = \setof{a_{n}}{(a_n,b) \in R_{n+1}}$. The intersection of $S_a, T_b$
is defined as all the pairs $(a_2, a_n)$ such that there is path from $a_2$ to
$a_n$. The sets $S_a$ and $T_b$ form
two families of sets, $\mR^S$ and $\mR^T$. 
Using this new definition of intersection, we can construct a tree structure
for the modified \GFSI\ problem on $\mR^S$ and $\mR^T$. The difference now
is what we do when we find a non-heavy set at some node of the tree; suppose 
w.l.o.g. that $S_a$ becomes light. Recall
that in this case, there are at most $\delta$ elements in the set. For each $a_2 \in S_a$,
we can now recursively use the compressed representation for the path query
$P_{n-1}$ to enumerate all paths with endpoints $a_2, b$. By induction, this enumeration
will have delay $O(\delta^{n-2})$. 
The total delay will be the product of the two delays, so $\delta \cdot \delta^{n-2} = \delta^{n-1}$.
Finally, observe that the space required is only $O(m^2/\delta^2)$.
\end{proof}

The space/delay tradeoff in this case becomes:
%
 $$ \textsf{space} \times \textsf{delay}^{2/(n-1)} = O(|D|^2).$$

In the general setting where $\bx_\sigma = \set{x_{i_1}, \dots, x_{i_r}}$ for
$i_1 < i_2 < \dots < i_r$, we observe that because of the structure of the path query,
we can enumerate the values of each ``segment" between $x_{i_j}$ and $x_{i_{j+1}}$  
independently of the values of the other segments. The enumeration for the segment  
between $x_{i}$ and $x_{i'}$ has
delay $O(\delta^{i'-i-1})$ and space $O(m^2/\delta^2)$. Thus, with space $O(m^2/\delta^2)$
we can achieve delay $O(\delta^{\ell-1})$, where $\ell$ is the largest distance between two
consecutive indexes in  $\bx_\sigma$. Notice that when $r \leq 1$, there is no segment, and
we can obtain constant delay with linear space. This is of course expected, since for $r=0$
we have the full enumeration query, which can be enumerated in constant delay because of
its acyclicity.

\subsection{Cycle Queries}

The final class of queries we will discuss is the class of {\em cycle queries}, which are 
CQs of the following form:
%
$$ C_n(x_1, \dots, x_n) = R_1(x_1, x_2), R_2(x_2, x_3), \dots, R_k(x_n, x_1).$$
%

We will consider the \pcq\ $(\set{x_1, x_2}, \set{x_3, \dots, x_n})$, and we will use it to obtain
a compressed representation for the full enumeration \pcq\ with the same space/delay tradeoff.

A simple first idea would be to use the compressed representation for $P_{n-1}$ as a black box.
This would give us delay $O(\delta^{n-2})$ with space $O(m^2/\delta^2)$. We show next how
to improve upon this first attempt.

\begin{proposition}
There exists a compressed representation of the cycle query $C_n$ that uses  space 
%
$$O(|D|^{2-1/(n-1)}/\delta^{2/(n-1)})$$
and can be used to enumerate the full enumeration \pcq\ 
with delay $O(\delta)$.
\end{proposition}

\begin{proof}
Consider the recursive compressed representation we constructed for the path query $P_{n-1}$.
At the first level of the recursion, we used the tree data structure for \GFSI\ without using any bound
on the number of queries $\mQ$. But in this case we know that the number of queries we can have
is at most $m$. In this case, we know from Theorem~\ref{thm:fksi} that we can get $O(\delta_1)$ delay
with space $O(m^{3/2}/\delta_1)$. The recursive call will to $P_{n-2}$ will now require space
$O(m^2/\delta_2^2)$ with delay $O(\delta_2^{n-3})$. The total delay is $\delta = \delta_1 \cdot \delta_2^{n-3}$,
and the total space is
%
$$S = \frac{m^{3/2}}{\delta_1} + \frac{m^2}{\delta_2^2}.$$
%
We can optimize the space/delay tradeoff by choosing $\delta_1, \delta_2$ such that
$m^2/\delta_2^2 = m^{3/2}/\delta_1$, so $\delta_1 = \delta_2^2/m^{1/2}$. Consequently, we obtain
delay $\delta = \delta_2^{n-1}/m^{1/2}$ with space $O(m^2/\delta_2^2) = O(m^{2-1/(n-1)}/\delta^{2/(n-1)})$.
\end{proof}

Notice that this recovers our result for the space/delay tradeoff for the triangle query. The space/delay 
tradeoff in general can be stated as:
%
 $$ \textsf{space} \times \textsf{delay}^{2/(n-1)} = O(|D|^{2-1/(n-1)}).$$
%
For $\delta=O(1)$, we obtain that the space requirement is only $O(|D|^{2-1/(n-1)})$. 
This result is surprising, since the fractional hypertree-width of a cycle query for $k \geq 4$ is equal to 2. 
Thus, the factorized representation would achieve constant delay with space $O(|D|^2)$. It turns out that
we can achieve the same delay by using less space.


%\subsection{Compressing Squares}
%
%We next consider the square query $C_4$. If all relations have the same size, i.e. $|R_i| = m$, we know that the worst-case output size is $O(m^2)$.
%
%\begin{lemma}
%The square query $C_4$ admits a compression scheme with size $O(m^2/\delta)$ and delay  $O(\delta)$, where $m = |R_i|$ for every $i=1,2,3,4$.
%\end{lemma}
%
%\begin{proof}
%The idea works as follows. Suppose that we want to achieve a delay of $O(m)$. Then, during the compression phase, we need to compute which tuples $R_1(a_1,a_2)$ participate in an output tuple (this needs size $O(m)$). We also compute two hash table for relations $R_2, R_4$. During decompression, we iterate over every tuple $R_1(a_1,a_2)$ that belongs in some output; then, we  go over every tuple $R_3(a_3, a_4)$, and check whether $(a_2, a_3)$ and $(a_4, a_1)$ are tuples in $R_2, R_4$ respectively. Since we can check this in constant time by querying the hash table, the delay we get is $\delta = O(m)$  (we know by construction that some tuple from $R_3$ will form a triangle with $(a_1,a_2)$).
%
%In order to achieve a smaller delay $\delta$, we need to store more information per tuple $R_1(a_1,a_2)$. Suppose we have ordered the tuples in $R_3$ according to some fixed order. We split then $R_3$ into $m/\delta$ subsets of size $\delta$; for each of these subsets, and each of the tuples $R_1(a_1,a_2)$, we store in the compressed result whether some tuple from the $i$-th subset participates in an output tuple with $(a_1, a_2)$ or not. This needs size $O(m^2/\delta)$ to be stored. In the decompression phase, for each tuple $R_1(a_1,a_2)$, we can skip the subsets of $R_3$ that have no participating tuple in an output; hence, the delay will now be $O(\delta)$, since each subset of $R_3$ has $\delta$ tuples. 
%\end{proof}


%The compression scheme for $C_k$ works as follows. We first fix a threshold $\beta$ that 
%we will show how to pick later in the analysis
%The first step is to remove from the database
%any tuples that do not participate in any $k$-cycle, and order each relation $R_j$ in
%lexicographic order. Also, we split each $R_j$ into $m_j/\beta$ intervals of size $\beta$.
%Then, for each pair $i, j$ we will construct a
%data structure $\mathcal{D}_{ij}$ as follows. Consider the relation
%$R_j(x_j, x_{j+1})$. For each value $a$ of $x_i$ with degree $\geq \beta$ in $R_i(x_i, x_{i+1})$, we  store in the compressed result whether some tuple from the $i$-th interval participates in an output cycle with $a$. Since there are at most $m_j/\beta$ such intervals, we need to remember at most $m_j/\beta$ data. Additionally, since there are at most $m_i/\beta$ value with degree $\geq \beta$, the total space needed by this data structure is $O(m_i  m_j / \beta^2)$.
%
%Let us say that an output cycle $C_k(a_1, a_2, \dots, a_k)$ is $i$-heavy (for $i=1, \dots, k, k+1$) if $i = \arg \min_j \{ d_{R_j}(a_j ) \geq \beta \}$. In a $k+1$-heavy cycle, all values have degree $< \beta$. Also notice that no output cycle can be both $i$-heavy and $j$-heavy for $i \neq j$.
%
%We can now describe the decompression algorithm. 
%The algorithm works in $k+1$ phases, where in phase $i$ it outputs all $i$-heavy cycles. We first start with the $k+1$-phase, which is the easiest to describe. We iterate over all edges $R_k(a_k, a_1)$ such that $a_1$ has degree $\leq \beta$ in $R_1$ and the edge belongs in a $k+1$-heavy cycle. For each $a_1$, we find all $R_1(a_1, a_2)$ such that $d_{R_2}(a_2) \leq \beta$, and so on.  After we have reached some $a_{k-1}$, we can simply check whether $R_{k-1}(a_{k-1}, a_k)$ in constant time. Since at each point we look at $\beta$ possible values, and we know for sure that $R_k(a_k, a_1)$ exists in an $k+1$-heavy cycle, the delay will be at most $\delta = O(\beta^{k-2})$. 
%
%Now consider the $i$-phase for $i \leq k$. To simplify the presentation, assume that $i=k$. In this phase, we iterate over all edges $R_k(a_k, a_1)$ such that $a_k$ has degree $\geq  \beta$ in $R_k$ and the edge belongs in a $k$-heavy cycle. Now, to find the next $a_2$, we will use the data structure $\mathcal{D}_{k1}$. Since we know which intervals we need to visit, we are certain than by iterating over at most $\beta$ values in a valid interval, we will discover a cycle. We do a similar thing for $a_3, a_4$, and so on. When we have reached $a_{k-1}$, we can  again simply check whether $R_{k-1}(a_{k-1}, a_k)$ in constant time. The delay for this phase is thus again $\delta = O(\beta^{k-2})$.
%
%Thus, if we want to achieve a delay $\delta$, we need to choose threshold $\delta = \beta^{1/(k-2)}$, in which case our compression algorithm requires size $O(|D|^2/\delta^{2/(k-2)})$.




